On the Location of the Minimizer of the Sum of Two Strongly Convex Functions

The problem of finding the minimizer of a sum of convex functions is central to the field of distributed optimization. Thus, it is of interest to understand how that minimizer is related to the properties of the individual functions in the sum. In this paper, we provide an upper bound on the region containing the minimizer of the sum of two strongly convex functions. We consider two scenarios with different constraints on the upper bound of the gradients of the functions. In the first scenario, the gradient constraint is imposed on the location of the potential minimizer, while in the second scenario, the gradient constraint is imposed on a given convex set in which the minimizers of two original functions are embedded. We characterize the boundaries of the regions containing the minimizer in both scenarios.

==> (ArXiv) On the Location of the Minimizer of the Sum of%5C%5C Two Strongly Convex Functions/intro.tex <==
\section{Introduction}
The problem of distributed optimization arises in a variety of applications, including machine learning \cite{Ma09, Shalev11, Boyd11ADMM, Sayed14}, control of large-scale systems \cite{DistOptGrid14, Li2011optimal}, and cooperative robotic systems \cite{Schwager09,hosseini2013online, Montijano14,hosseini2014online,Zhu15}. In such problems, each node in a network has access to a local convex function (e.g., representing certain data available at that node), and all nodes are required to calculate the minimizer of the sum of the local functions.  There is a significant literature on distributed algorithms that allow the nodes to achieve this objective \cite{JNT-DPB-MA:86, Nedic10constrained,BJ-MR-MJ:09,MZ-SM:12,JW-NE:11, BG-JC:14-tac, AN-AO:15-tac}.  The local functions in the above settings are typically assumed to be private to the nodes.  However, there are certain common assumptions that are made about the characteristics of such functions, including strong convexity and bounds on the gradients (e.g., due to minimization over a convex set).  

In certain applications, it may be of interest to determine a region where the minimizer of the sum of the functions can be located, given only the minimizers of the local functions, their strong convexity parameters, and the bound on their gradients (either at the minimizer or at the boundaries of a convex constraint set).  For example, when the network contains malicious nodes that do not follow the distributed optimization algorithm, one cannot guarantee that all nodes calculate the true minimizer.  Instead, one must settle for algorithms that allow the non-malicious nodes to converge to a certain region \cite{sundaram2016secure,LS-NV:15}.  In such situations, knowing the region where the minimizer can lie would allow us to evaluate the efficacy of such resilient distributed optimization algorithms.  Similarly, suppose that the true functions at some (or all) nodes are not known (e.g., due to noisy data, or if the nodes obfuscate their functions due to privacy concerns).  A key question in such scenarios is to determine how far the minimizer of the sum of the true functions can be from the minimizer calculated from the noisy (or obfuscated) functions.  The region containing all possible minimizers of the sum of functions (calculated using only their local minimizers, convexity parameters, and bound on the gradients) would provide the answer to this question.  

When the local functions $f_i$ at each node $v_i$ are single dimensional (i.e., $f_i: \mathbb{R} \rightarrow \mathbb{R}$), and strongly convex, it is easy to see that the minimizer of the sum of functions must be in the interval bracketed by the smallest and largest minimizers of the local functions.  This is because the gradients of all the functions will have the same sign outside that region, and thus cannot sum to zero.  However, a similar characterization of the region containing the minimizer of multidimensional functions is lacking in the literature, and is significantly more challenging to obtain.  For example, the conjecture that the minimizer of a sum of convex functions is in the convex hull of their local minimizers can be easily disproved via simple examples; consider $f_1(x,y) = x^2 - xy + \frac{1}{2} y^2$ and $f_2(x,y) = x^2 + xy + \frac{1}{2} y^2 -4x -2y$ with minimizers $(0,0)$ and $(2,0)$ respectively, whose sum has minimizer $(1, 1)$. Thus, in this paper, {\bf our goal is to take a step toward characterizing the region containing the minimizer of a sum of strongly convex functions.}  Specifically, we focus on characterizing this region for the sum of {\it two} strongly convex functions under various assumptions on their gradients (as described in the next section).  As we will see, the analysis is significantly complicated even for this scenario.  Nevertheless, we obtain such a region and gain insights that could potentially be leveraged in future work to tackle the sum of multiple functions.

